3D Trajectory Reconstruction of Dynamic Objects Using Planarity Constraints

We present a method to reconstruct the three-dimensional trajectory of a moving instance of a known object category in monocular video data. We track the two-dimensional shape of objects on pixel level exploiting instance-aware semantic segmentation techniques and optical flow cues. We apply Structure from Motion techniques to object and background images to determine for each frame camera poses relative to object instances and background structures. By combining object and background camera pose information, we restrict the object trajectory to a one-parameter family of possible solutions. We compute a ground representation by fusing background structures and corresponding semantic segmentations. This allows us to determine an object trajectory consistent to image observations and reconstructed environment model. Our method is robust to occlusion and handles temporarily stationary objects. We show qualitative results using drone imagery. Due to the lack of suitable benchmark datasets we present a new dataset to evaluate the quality of reconstructed three-dimensional object trajectories. The video sequences contain vehicles in urban areas and are rendered using the path-tracing render engine Cycles to achieve realistic results. We perform a quantitative evaluation of the presented approach using this dataset. Our algorithm achieves an average reconstruction-to-ground-truth distance of 0.31 meter.

==> experiments_introduction.tex <==
We perform a set of qualitative and quantitative evaluations using real drone footage and virtual generated drone flights.

\begin{figure*}
	% use the subfloat package (not subfigure or subfig)
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width=\subfigureWidthFourColumns]{images/real_images/frame00000.jpg}
		\caption{Input Frame 0}
		\label{fig:input_frame_0}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthFourColumns]{images/real_images/frame00050.jpg}
		\caption{Input Frame 50}
		\label{fig:input_frame_50}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthFourColumns]{images/real_images/frame00100.jpg}
		\caption{Input Frame 100}
		\label{fig:input_frame_100}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthFourColumns]{images/real_images/frame00150.jpg}
		\caption{Input Frame 150}
		\label{fig:input_frame_150}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthFourColumns]{images/real_images/frame00200.jpg}
		\caption{Input Frame 200}
		\label{fig:input_frame_200}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthFourColumns]{images/real_images/frame00250.jpg}
		\caption{Input Frame 250}
		\label{fig:input_frame_250}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthFourColumns]{images/real_images/real_traj_45_deg.jpg}
		\caption{Reconstructed Trajectory (Side View)}
		\label{fig:real_trajectory_side_view}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthFourColumns]{images/real_images/real_traj_top_view.jpg}
		\caption{Reconstructed Trajectory (Top View)}
		\label{fig:real_trajectory_top_view}
	\end{subfigure}
	\caption{Car Trajectory Reconstruction using 250 frames captured by a DJI drone.}
	\label{fig:trajectory_reconstruction_real}
\end{figure*}

Fig. \ref{fig:trajectory_reconstruction_real} shows the reconstruction of a car motion trajectory using the imagery of an DJI drone. The sequence contained 250 frames with a resolution of 1920 x 1080 pixels.
\begin{figure*}
	% use the subfloat package (not subfigure or subfig)
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/trajectory_gt.jpg}
		\caption{Ground Truth Object Path}
		\label{fig:evaluation:quantitative_evaluation_object_path}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/model_in_scene.jpg}
		\caption{Object Model in Blender}
		\label{fig:evaluation:quantitative_evaluation_object_model}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/frame00039_orig.jpg}
		\caption{Rendered Scene}
		\label{fig:evaluation:quantitative_evaluation_rendered_scene}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/frame00039_object_seg.jpg}
		\caption{Object Segmentation}
		\label{fig:evaluation:quantitative_evaluation_object_seg}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/frame00039_background_seg.jpg}
		\caption{Background Segmentation}
		\label{fig:evaluation:quantitative_evaluation_background_sec}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/frame00039_ground_seg.jpg}
		\caption{Ground Segmentation}
		\label{fig:evaluation:quantitative_evaluation_ground_sec}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/object_reconstruction.jpg}
		\caption{Object Reconstruction}
		\label{fig:evaluation:quantitative_evaluation_obj_rec}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/background_reconstruction.jpg}
		\caption{Background Reconstruction}
		\label{fig:evaluation:quantitative_evaluation_background_rec}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/trajectory_reconstruction1.jpg}
		\caption{Reconstructed Trajectory}
		\label{fig:evaluation:quantitative_evaluation_overlay_reconstructed_trajectory}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/trajectory_reconstruction2.jpg}
		\caption{Reconstructed Object Trajectory}
		\label{fig:evaluation:quantitative_evaluation_overlay_3_top}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/trajectory_ground_truth_with_reconstruction1.jpg}
		\caption{Ground Truth Model at Different Frames Overlayed With Reconstruction}
		\label{fig:evaluation:quantitative_evaluation_ground_truth_with_points_top_1}
	\end{subfigure}
	\begin{subfigure}[t]{\subfigureWidthFourColumns}
		\includegraphics[width = \subfigureWidthThreeColumns]{images/quant_evaluation/trajectory_ground_truth_with_reconstruction2.jpg}
		\caption{Ground Truth Model at Different Frames Overlayed With Reconstruction}
		\label{fig:evaluation:quantitative_evaluation_ground_truth_with_points_topaa_2a}
	\end{subfigure}
	\caption{Car Trajectory Reconstruction using 250 frames captured by a DJI drone.}
	\label{fig:evaluation:quantitative_evaluation}
	% ground truth path, image with model from scene, rendered image, 
	% object image, background image, ground image
	% object reconstr, background rec, ground rec
	% 1-parameter family, reconstructed trajec1, reconstructed traj2 
	% scene with points, ground truth with points1, ground truth with points2
	% = 15 images
\end{figure*}


Fig. \ref{fig:evaluation:quantitative_evaluation} shows an example of our quantitative evaluation using the virtual object trajectory dataset. Fig. \ref{fig:evaluation:quantitative_evaluation_overlay} shows the object point cloud transformed into the virtual world coordinate frame system. Fig. \ref{fig:evaluation:quantitative_evaluation_distance_values} shows the distance values of transformed points and virtual model.

\cite{Bullinger2016}

\cite{Bodensteiner_2015_ICCV_Workshops}

%Sturm et al. \cite{Sturm2012} presented a metric called Absolute Trajectory Error (ATE) to compare two trajectories, possibly defined in different coordinate frames. Their implementation requires a scale ratio between these coordinate frames.

% TODO \cite{Chhaya2016} 

==> methods_scale_estimation_using_constant_distance_non_planar.tex <==




